Semantic Matching of Documents from Heterogeneous Collections: A Simple and Transparent Method for Practical Applications

We present a very simple, unsupervised method for the pairwise matching of documents from heterogeneous collections. We demonstrate our method with the Concept-Project matching task, which is a binary classification task involving pairs of documents from heterogeneous collections. Although our method only employs standard resources without any domain- or task-specific modifications, it clearly outperforms the more complex system of the original authors. In addition, our method is transparent, because it provides explicit information about how a similarity score was computed, and efficient, because it is based on the aggregation of (pre-computable) word-level similarities.

==> tuning.tex <==
\section{Tuning}

\begin{table*}
\begin{tiny}
\begin{tabular}{l|l|l|l}
\multicolumn{4}{l}{\textbf{\begin{tiny}-avgcosine-none-none-unfoldedidftokens-none-algo:glove;dataset:840b;dims:300;fold:0;norm:none;unit:token\end{tiny}}}\\
\textbf{TS} & \textbf{P} & \textbf{R} & \textbf{F} \\
$0.3\_[]\_[]$ & $0.55102$ & $0.98182$ & $\textbf{0.70588}$\\
\hline
$0.37500000000000006\_[]\_[]$ & $0.55670$ & $0.98182$ & $\textbf{0.71053}$\\
\hline
$0.3950000000000001\_[]\_[]$ & $0.56250$ & $0.98182$ & $\textbf{0.71523}$\\
\hline
$0.4150000000000001\_[]\_[]$ & $0.56842$ & $0.98182$ & $\textbf{0.72000}$\\
\hline
$0.4450000000000001\_[]\_[]$ & $0.57447$ & $0.98182$ & $\textbf{0.72483}$\\
\hline
$0.4500000000000001\_[]\_[]$ & $0.58065$ & $0.98182$ & $\textbf{0.72973}$\\
\hline
$0.46500000000000014\_[]\_[]$ & $0.58696$ & $0.98182$ & $\textbf{0.73469}$\\
\hline
$0.47500000000000014\_[]\_[]$ & $0.59341$ & $0.98182$ & $\textbf{0.73973}$\\
\hline
$0.48500000000000015\_[]\_[]$ & $0.60000$ & $0.98182$ & $\textbf{0.74483}$\\
\hline
$0.5000000000000002\_[]\_[]$ & $0.60674$ & $0.98182$ & $\textbf{0.75000}$\\
\hline
$0.5100000000000002\_[]\_[]$ & $0.62069$ & $0.98182$ & $\textbf{0.76056}$\\
\hline
$0.5200000000000002\_[]\_[]$ & $0.62791$ & $0.98182$ & $\textbf{0.76596}$\\
\hline
$0.5300000000000002\_[]\_[]$ & $0.63529$ & $0.98182$ & $\textbf{0.77143}$\\
\hline
$0.5350000000000001\_[]\_[]$ & $0.64286$ & $0.98182$ & $\textbf{0.77698}$\\
\hline
$0.5600000000000003\_[]\_[]$ & $0.65854$ & $0.98182$ & $\textbf{0.78832}$\\
\hline
$0.5650000000000002\_[]\_[]$ & $0.67500$ & $0.98182$ & $\textbf{0.80000}$\\
\hline
$0.5900000000000003\_[]\_[]$ & $0.68354$ & $0.98182$ & $\textbf{0.80597}$\\
\hline
$0.5950000000000002\_[]\_[]$ & $0.69231$ & $0.98182$ & $\textbf{0.81203}$\\
\hline
$0.6000000000000003\_[]\_[]$ & $0.70130$ & $0.98182$ & $\textbf{0.81818}$\\
\hline
$0.6050000000000002\_[]\_[]$ & $0.71053$ & $0.98182$ & $\textbf{0.82443}$\\
\hline
$0.6100000000000003\_[]\_[]$ & $0.72000$ & $0.98182$ & $\textbf{0.83077}$\\
\hline
$0.6250000000000002\_[]\_[]$ & $0.73611$ & $0.96364$ & $\textbf{0.83465}$\\
\hline
$0.6300000000000003\_[]\_[]$ & $0.74648$ & $0.96364$ & $\textbf{0.84127}$\\
\hline
$0.6350000000000002\_[]\_[]$ & $0.75714$ & $0.96364$ & $\textbf{0.84800}$\\
\hline
$0.6400000000000003\_[]\_[]$ & $0.76812$ & $0.96364$ & $\textbf{0.85484}$\\
\hline
$0.6450000000000002\_[]\_[]$ & $0.77941$ & $0.96364$ & $\textbf{0.86179}$\\
\hline
$0.6500000000000004\_[]\_[]$ & $0.80303$ & $0.96364$ & $\textbf{0.87603}$\\
\hline
$0.6600000000000004\_[]\_[]$ & $0.82540$ & $0.94545$ & $\textbf{0.88136}$\\
\hline
$0.6950000000000003\_[]\_[]$ & $0.87500$ & $0.89091$ & $\textbf{0.88288}$\\
\hline
$0.7150000000000003\_[]\_[]$ & $0.92308$ & $0.87273$ & $\textbf{0.89720}$\\
\hline
\end{tabular}
\end{tiny}
\end{table*}

\begin{table*}
\begin{tiny}
\begin{tabular}{l|l|l|l}
\multicolumn{4}{l}{\textbf{\begin{tiny}-avgcosine-none-none-unfoldedidftypes-none-algo:glove;dataset:840b;dims:300;fold:0;norm:none;unit:token\end{tiny}}}\\
\textbf{TS} & \textbf{P} & \textbf{R} & \textbf{F} \\
$0.3\_[]\_[]$ & $0.55102$ & $0.98182$ & $\textbf{0.70588}$\\
\hline
$0.4100000000000001\_[]\_[]$ & $0.55670$ & $0.98182$ & $\textbf{0.71053}$\\
\hline
$0.4500000000000001\_[]\_[]$ & $0.56250$ & $0.98182$ & $\textbf{0.71523}$\\
\hline
$0.46500000000000014\_[]\_[]$ & $0.56842$ & $0.98182$ & $\textbf{0.72000}$\\
\hline
$0.47500000000000014\_[]\_[]$ & $0.57447$ & $0.98182$ & $\textbf{0.72483}$\\
\hline
$0.48000000000000015\_[]\_[]$ & $0.58065$ & $0.98182$ & $\textbf{0.72973}$\\
\hline
$0.5200000000000002\_[]\_[]$ & $0.58696$ & $0.98182$ & $\textbf{0.73469}$\\
\hline
$0.5250000000000001\_[]\_[]$ & $0.59341$ & $0.98182$ & $\textbf{0.73973}$\\
\hline
$0.5300000000000002\_[]\_[]$ & $0.60000$ & $0.98182$ & $\textbf{0.74483}$\\
\hline
$0.5750000000000002\_[]\_[]$ & $0.60674$ & $0.98182$ & $\textbf{0.75000}$\\
\hline
$0.5800000000000003\_[]\_[]$ & $0.61364$ & $0.98182$ & $\textbf{0.75524}$\\
\hline
$0.5900000000000003\_[]\_[]$ & $0.62069$ & $0.98182$ & $\textbf{0.76056}$\\
\hline
$0.5950000000000002\_[]\_[]$ & $0.62791$ & $0.98182$ & $\textbf{0.76596}$\\
\hline
$0.6000000000000003\_[]\_[]$ & $0.64286$ & $0.98182$ & $\textbf{0.77698}$\\
\hline
$0.6050000000000002\_[]\_[]$ & $0.65854$ & $0.98182$ & $\textbf{0.78832}$\\
\hline
$0.6100000000000003\_[]\_[]$ & $0.66667$ & $0.98182$ & $\textbf{0.79412}$\\
\hline
$0.6150000000000002\_[]\_[]$ & $0.67500$ & $0.98182$ & $\textbf{0.80000}$\\
\hline
$0.6300000000000003\_[]\_[]$ & $0.68354$ & $0.98182$ & $\textbf{0.80597}$\\
\hline
$0.6450000000000002\_[]\_[]$ & $0.69231$ & $0.98182$ & $\textbf{0.81203}$\\
\hline
$0.6550000000000002\_[]\_[]$ & $0.72000$ & $0.98182$ & $\textbf{0.83077}$\\
\hline
$0.6750000000000003\_[]\_[]$ & $0.73611$ & $0.96364$ & $\textbf{0.83465}$\\
\hline
$0.7100000000000004\_[]\_[]$ & $0.78125$ & $0.90909$ & $\textbf{0.84034}$\\
\hline
$0.7550000000000003\_[]\_[]$ & $0.86538$ & $0.81818$ & $\textbf{0.84112}$\\
\hline
\end{tabular}
\end{tiny}
\end{table*}

\begin{table*}
\begin{tiny}
\begin{tabular}{l|l|l|l}
\multicolumn{4}{l}{\textbf{\begin{tiny}-avgcosine-none-none-unfoldedtokens-none-algo:glove;dataset:840b;dims:300;fold:0;norm:none;unit:token\end{tiny}}}\\
\textbf{TS} & \textbf{P} & \textbf{R} & \textbf{F} \\
$0.3\_[]\_[]$ & $0.55102$ & $0.98182$ & $\textbf{0.70588}$\\
\hline
$0.4050000000000001\_[]\_[]$ & $0.55670$ & $0.98182$ & $\textbf{0.71053}$\\
\hline
$0.46500000000000014\_[]\_[]$ & $0.56250$ & $0.98182$ & $\textbf{0.71523}$\\
\hline
$0.5100000000000002\_[]\_[]$ & $0.56842$ & $0.98182$ & $\textbf{0.72000}$\\
\hline
$0.5150000000000001\_[]\_[]$ & $0.58065$ & $0.98182$ & $\textbf{0.72973}$\\
\hline
$0.5200000000000002\_[]\_[]$ & $0.58696$ & $0.98182$ & $\textbf{0.73469}$\\
\hline
$0.5500000000000003\_[]\_[]$ & $0.59341$ & $0.98182$ & $\textbf{0.73973}$\\
\hline
$0.5650000000000002\_[]\_[]$ & $0.60000$ & $0.98182$ & $\textbf{0.74483}$\\
\hline
$0.5700000000000003\_[]\_[]$ & $0.60674$ & $0.98182$ & $\textbf{0.75000}$\\
\hline
$0.5750000000000002\_[]\_[]$ & $0.61364$ & $0.98182$ & $\textbf{0.75524}$\\
\hline
$0.5800000000000003\_[]\_[]$ & $0.62069$ & $0.98182$ & $\textbf{0.76056}$\\
\hline
$0.5850000000000002\_[]\_[]$ & $0.62791$ & $0.98182$ & $\textbf{0.76596}$\\
\hline
$0.6050000000000002\_[]\_[]$ & $0.63529$ & $0.98182$ & $\textbf{0.77143}$\\
\hline
$0.6250000000000002\_[]\_[]$ & $0.64286$ & $0.98182$ & $\textbf{0.77698}$\\
\hline
$0.6300000000000003\_[]\_[]$ & $0.65060$ & $0.98182$ & $\textbf{0.78261}$\\
\hline
$0.6400000000000003\_[]\_[]$ & $0.66667$ & $0.98182$ & $\textbf{0.79412}$\\
\hline
$0.6450000000000002\_[]\_[]$ & $0.67500$ & $0.98182$ & $\textbf{0.80000}$\\
\hline
$0.6500000000000004\_[]\_[]$ & $0.68354$ & $0.98182$ & $\textbf{0.80597}$\\
\hline
$0.6550000000000002\_[]\_[]$ & $0.69231$ & $0.98182$ & $\textbf{0.81203}$\\
\hline
$0.6700000000000004\_[]\_[]$ & $0.72603$ & $0.96364$ & $\textbf{0.82812}$\\
\hline
$0.6750000000000003\_[]\_[]$ & $0.73611$ & $0.96364$ & $\textbf{0.83465}$\\
\hline
$0.6800000000000004\_[]\_[]$ & $0.75714$ & $0.96364$ & $\textbf{0.84800}$\\
\hline
$0.6850000000000003\_[]\_[]$ & $0.78788$ & $0.94545$ & $\textbf{0.85950}$\\
\hline
$0.6900000000000004\_[]\_[]$ & $0.81250$ & $0.94545$ & $\textbf{0.87395}$\\
\hline
\end{tabular}
\end{tiny}
\end{table*}

\begin{table*}
\begin{tiny}
\begin{tabular}{l|l|l|l}
\multicolumn{4}{l}{\textbf{\begin{tiny}-avgcosine-none-none-unfoldedtypes-none-algo:glove;dataset:840b;dims:300;fold:0;norm:none;unit:token\end{tiny}}}\\
\textbf{TS} & \textbf{P} & \textbf{R} & \textbf{F} \\
$0.3\_[]\_[]$ & $0.55102$ & $0.98182$ & $\textbf{0.70588}$\\
\hline
$0.4450000000000001\_[]\_[]$ & $0.55670$ & $0.98182$ & $\textbf{0.71053}$\\
\hline
$0.5100000000000002\_[]\_[]$ & $0.56250$ & $0.98182$ & $\textbf{0.71523}$\\
\hline
$0.5350000000000001\_[]\_[]$ & $0.56842$ & $0.98182$ & $\textbf{0.72000}$\\
\hline
$0.5450000000000002\_[]\_[]$ & $0.57447$ & $0.98182$ & $\textbf{0.72483}$\\
\hline
$0.5650000000000002\_[]\_[]$ & $0.58065$ & $0.98182$ & $\textbf{0.72973}$\\
\hline
$0.5800000000000003\_[]\_[]$ & $0.58696$ & $0.98182$ & $\textbf{0.73469}$\\
\hline
$0.6050000000000002\_[]\_[]$ & $0.59341$ & $0.98182$ & $\textbf{0.73973}$\\
\hline
$0.6100000000000003\_[]\_[]$ & $0.60000$ & $0.98182$ & $\textbf{0.74483}$\\
\hline
$0.6250000000000002\_[]\_[]$ & $0.60674$ & $0.98182$ & $\textbf{0.75000}$\\
\hline
$0.6450000000000002\_[]\_[]$ & $0.61364$ & $0.98182$ & $\textbf{0.75524}$\\
\hline
$0.6550000000000002\_[]\_[]$ & $0.62069$ & $0.98182$ & $\textbf{0.76056}$\\
\hline
$0.6600000000000004\_[]\_[]$ & $0.63529$ & $0.98182$ & $\textbf{0.77143}$\\
\hline
$0.6650000000000003\_[]\_[]$ & $0.64286$ & $0.98182$ & $\textbf{0.77698}$\\
\hline
$0.6800000000000004\_[]\_[]$ & $0.65432$ & $0.96364$ & $\textbf{0.77941}$\\
\hline
$0.6850000000000003\_[]\_[]$ & $0.66250$ & $0.96364$ & $\textbf{0.78519}$\\
\hline
$0.6950000000000003\_[]\_[]$ & $0.67949$ & $0.96364$ & $\textbf{0.79699}$\\
\hline
$0.7000000000000004\_[]\_[]$ & $0.69737$ & $0.96364$ & $\textbf{0.80916}$\\
\hline
$0.7250000000000003\_[]\_[]$ & $0.73239$ & $0.94545$ & $\textbf{0.82540}$\\
\hline
$0.7300000000000004\_[]\_[]$ & $0.75362$ & $0.94545$ & $\textbf{0.83871}$\\
\hline
$0.7350000000000003\_[]\_[]$ & $0.76471$ & $0.94545$ & $\textbf{0.84553}$\\
\hline
\end{tabular}
\end{tiny}
\end{table*}

